Hierarchical Pre-training for Sequence Labelling in Spoken Dialog

Sequence labelling tasks like Dialog Act and Emotion/Sentiment identification are a key component of spoken dialog systems. In this work, we propose a new approach to learn generic representations adapted to spoken dialog, which we evaluate on a new benchmark we call Sequence labellIng evaLuatIon benChmark fOr spoken laNguagE benchmark (\texttt{SILICONE}). \texttt{SILICONE} is model-agnostic and contains 10 different datasets of various sizes. We obtain our representations with a hierarchical encoder based on transformer architectures, for which we extend two well-known pre-training objectives. Pre-training is performed on OpenSubtitles: a large corpus of spoken dialog containing over $2.3$ billion of tokens. We demonstrate how hierarchical encoders achieve competitive results with consistently fewer parameters compared to state-of-the-art models and we show their importance for both pre-training and fine-tuning.

==> evaluation.tex <==
\subsection{Related Work}
Sequence labelling tasks for spoken dialog mainly involve two different types of labels: \texttt{DA} and \texttt{E/S}. Early work has tackled the sequence labelling problem as an independent classification of each utterance. Deep neural network models that currently achieve the best results~\cite{bayesian_dialog,svm_dialog,hmm_dialog} model both contextual dependencies between utterances~\cite{colombo2020guiding,concurrent_mrda} and labels~\cite{crf_chen,crf_kumar,crf_li}.

The aforementioned methods require large corpora to train models from scratch, such as: Switchboard Dialog Act (\texttt{SwDA})~\cite{datase_swda},  Meeting Recorder Dialog Act (\texttt{MRDA})~\cite{dataset_mrda}, Daily Dialog Act~\cite{dataset_dailydialog}, HCRC Map Task Corpus~(\texttt{MT})~\cite{dataset_maptask}.
This makes harder their adoption to smaller datasets, such as: Loqui human-human dialogue corpus (\texttt{Loqui})~\cite{dataset_loquihuman}, BT Oasis Corpus (\texttt{Oasis})~\cite{dataset_gtoasis}, Multimodal Multi-Party Dataset (\texttt{MELD})~\cite{dataset_meld}, Interactive emotional dyadic motion capture database (\texttt{IEMO}), SEMAINE database (\texttt{SEM})~\cite{dataset_semaine}. 

\subsection{Presentation of \texttt{SILICONE}}
Despite the similarity between methods usually employed to tackle \texttt{DA} and \texttt{E/S} sequential classification, studies usually rely on a single type of label. Moreover, despite the variety of small or medium-sized labelled datasets, evaluation is usually done on the largest available corpora (e.g., \texttt{SwDA}, \texttt{MRDA}).
We introduce \texttt{SILICONE}, a collection of sequence labelling tasks, gathering both \texttt{DA} and \texttt{E/S} annotated datasets. \texttt{SILICONE} is built upon preexisting datasets which have been considered by the community as challenging and interesting.
Any model that is able to process multiple sequences as inputs and predict the corresponding labels can be evaluated on \texttt{SILICONE}. %\texttt{SILICONE} does not place any constraints on model architecture beyond the ability to process multiple sequence inputs and to make corresponding predictions of the desired label.
We especially include small-sized datasets, as we believe it will ensure that well-performing models are able to both distil substantial knowledge and adapt to different sets of labels without relying on a large number of examples.
%Small-size datasets included in our benchmark ensure that good performance should require a model to have both substantial knowledge and quickly adapt to new set of labels.
The description of the datasets composing the benchmark can be found in the following sections, while corpora statistics are gathered in~\autoref{tab:presentation_of_silicon}.
%\texttt{SILICONE} is the first benchmark to gather such a diversity of corpora. 
% - We design the benchmark such that good performance should require a model to have substantial knowledge and could adapt to small size dataset. Dataset composing the benchmark are introduced based on their size and can be found in the following sections and statistics are gathered in \autoref{tab:presentation_of_silicon}.
% on a pas dit qu'on fait les deux DA et S/E
%\textbf{(CHloe) dialogue level or multi-utterance level ? Caracteristiques specifiques du dialogue : le dialogue est une sequence de tours de parole avec des locuteurs differents. Chaque tour de parole contient une séquence de phrases.}
%In this section we describe pretraining corpus as well as downstream tasks composing the benchmark.
%contains small and large dataset
%As our pretraining task on OpenSubtitle aims at resulting in representation that are label-agnostic and can be fine-tuned it is critical to develop a new benchmark on which we can compare the different models. We introduce SILICONE a collection of sequence labelling tasks including dialog act, sentiment and emotion labels. SILICONE does not place any constraints on model architecture beyond the ability to process multiple sequences inputs and to make corresponding predictions of the desired label. SILICONE was not created from scratch; it relies on preexisting datasets because they have been agreed upon by the community as challenging and interesting. We design the benchmark such that good performance should require a model to have substantial knowledge and could adapt to small size dataset. 
%\textbf{Miscellous}
%Additionnal ideas, transfert learning task specifics, different sizes Underly the fact that we use corpus of different size. , split follow

\subsubsection{\texttt{DA} Datasets}

\noindent\textbf{Switchboard Dialog Act Corpus (\texttt{SwDA})} is a telephone speech corpus consisting  of two-sided telephone conversations with provided topics. This dataset includes additional features such as speaker id and topic information. The SOTA model, based on a seq2seq architecture with guided attention, reports an accuracy of $85.5\%$~\cite{colombo2020guiding} on the official split.

\noindent\textbf{ICSI MRDA Corpus (\texttt{MRDA})} has been introduced by~\citet{dataset_mrda}. It contains transcripts of multi-party meetings hand-annotated with \texttt{DA}. It is the second biggest dataset with around $110k$ utterances. The SOTA model reaches an accuracy of $92.2\%$ \cite{sota_swda_1} and uses Bi-LSTMs with attention as encoder as well as additional features, such as the topic of the transcript. 

\noindent\textbf{DailyDialog Act Corpus ({$\texttt{DyDA}_\texttt{a}$})} has been produced by~\citet{dataset_dailydialog}. It contains multi-turn dialogues, supposed to reflect daily communication by covering topics about daily life. The dataset is manually labelled with dialog act and emotions. It is the third biggest corpus of \texttt{SILICONE} with $102k$ utterances. The SOTA model reports an accuracy of $88.1\%$~\cite{sota_swda_1}, using Bi-LSTMs with attention as well as additional features.
We follow the official split introduced by the authors.

\noindent\textbf{HCRC MapTask Corpus (\texttt{MT})} has been introduced by~\cite{dataset_maptask}. To build this corpus, participants were asked to collaborate verbally by describing a route from a first participant’s map by using the map of another participant. This corpus is small ($27k$ utterances). As there is no standard train/dev/test split\footnote{We split according to the code in https://github.com/NathanDuran/Maptask-Corpus.} performances depends on the split. \citet{tran2017generative} make use of a Hierarchical LSTM encoder with a GRU decoder layer and achieves an accuracy of $65.9\%$.

\noindent\textbf{Bt Oasis Corpus (\texttt{Oasis})} contains the transcripts of live calls made to the BT and operator services. This corpus has been introduced by~\cite{dataset_gtoasis} and is rather small ($15k$ utterances). There is no standard train/dev/test split \footnote{We use a random split from https://github.com/NathanDuran/BT-Oasis-Corpus.} and few studies use this dataset. 

\subsubsection{\texttt{S/E} Datasets}
In \texttt{S/E} recognition for spoken language, there is no consensus on the choice the evaluation metric (e.g., \citet{weighted_preproc,weighted_no} use a weighted F-score while \citet{accuracy_fscore} report accuracy). For \texttt{SILICONE}, we choose to stay consistent with the \texttt{DA} research and thus follow~\citet{accuracy_fscore} by reporting the accuracy. Additionally, emotion/sentiment labels are neither merged nor prepossessed\footnote{Comparison with concurrent work is more difficult as system performance heavily depends on the number of classes and label processing varies across studies \cite{variability}.}.
%In \texttt{S/E} recognition for spoken language there is a high variability both in the preprocessing step for labels and for the choice of the evaluation metric. (e.g \citet{weighted_preproc,weighted_no} use a weighted F-score where \citet{accuracy_fscore} report accuracy). For \texttt{SILICONE} we choose to stay consistent with the current trend in \texttt{DA} research and thus follow \citet{accuracy_fscore} and report the accuracy. Additionally emotion/sentiment labels are not merged and not preprocessed. \\

\noindent\textbf{DailyDialog Emotion Corpus ($\texttt{DyDA}_\texttt{e}$)} has been previously introduced and contains eleven emotional labels. The SOTA model~\cite{de2019joint} is based on BERT with additional Valence Arousal and Dominance features and reaches an accuracy of 85\% on the official split.

\noindent\textbf{Multimodal EmotionLines Dataset (\texttt{MELD})} has been created by enhancing and extending EmotionLines dataset~\cite{emotion_lines} where multiple speakers participated in the dialogues. There are two types of annotations $\texttt{MELD}_\texttt{s}$ and  $\texttt{MELD}_\texttt{e}$: three sentiments (positive, negative and neutral) and seven emotions (anger, disgust, fear, joy,neutral, sadness and surprise). The SOTA model with text only is proposed by \citet{accuracy_fscore} and is inspired by quantum physics. On the official split, it is compared with a hierarchical bi-LSTM, which it beats with an accuracy of $61.9$\% ($\texttt{MELD}_\texttt{s}$) and $67.9$\% ($\texttt{MELD}_\texttt{e}$) against $60.8\%$ and $65.2$.

\noindent\textbf{IEMOCAP database (\texttt{IEMO})} is a multimodal database of ten speakers. It consists of dyadic sessions where actors perform improvisations or scripted scenarios. Emotion categories are: anger, happiness, sadness, neutral, excitement, frustration, fear, surprise, and other. There is no official split on this dataset. One proposed model is built with bi-LSTMs and achieves $35.1\%$, with text only \cite{accuracy_fscore}.

\noindent\textbf{SEMAINE database (\texttt{SEM})} comes from the Sustained Emotionally coloured Machine human Interaction using Nonverbal Expression project~\cite{dataset_semaine}. This dataset has been annotated on three sentiments labels: positive, negative and neutral by \citet{barriere2018attitude}. It is built on Multimodal Wizard of Oz experiment where participants held conversations with an operator who adopted various roles designed to evoke emotional reactions. There is no official split on this dataset.
\begin{table*}
\begin{center}
\resizebox{.7\textwidth}{!}{ \begin{tabular}{c  c c c c c c c} 
 \hline
 Corpus  & $\lvert Train \rvert$ & $\lvert Val \rvert$ & $\lvert Test \rvert$ & Utt.& $\lvert Labels \rvert$ &Task& Utt./\lvert Labels \rvert \\ 
  \hline
  \texttt{SwDA}$^\star$  &  1k  & 100 & 11 & 200k   & 42 & \texttt{DA} & 4.8k\\

  \texttt{MRDA}$^\star$ &  56 & 6 &  12 &110k& 5& \texttt{DA} & 2.6k\\
      $\texttt{DyDA}_\texttt{a}$&  11k  & 1k & 1k & 102k  & 4 & \texttt{DA}& 25.5k \\
  \texttt{MT}$^\star$ &  121 & 22 & 25 &  36k & 12& \texttt{DA} & 3k\\
  \texttt{Oasis}$^\star$ &  508 & 64 & 64 & 15k & 42 & \texttt{DA} & 357\\
 \hline
    $\texttt{DyDA}_\texttt{e}$ &   11k  & 1k & 1k & 102k  & 7 &\texttt{E}&2.2k \\
    $\texttt{MELD}_\texttt{s}$$^\star$ &  934 & 104  &  280 & 13k  & 3 & \texttt{S} & 4.3k\\
        $\texttt{MELD}_\texttt{e}$$^\star$& 934 & 104  &  280 & 13k  & 7 & \texttt{S} & 1.8k\\
    \texttt{IEMO}&  108 & 12 & 31 & 10k & 6 & \texttt{E}&1.7k\\

      \texttt{SEM}  & 62 & 7 & 10 & 5,6k & 3 & \texttt{S}& 1.9k\\

\end{tabular}}
\end{center}

\caption{Statistics of datasets composing  \texttt{SILICONE}. \texttt{E} stands for emotion label and \texttt{S} for sentiment label; $^\star$ stands for datasets with available official split. Sizes of Train, Val and Test are given in number of conversations. }\label{tab:presentation_of_silicon}
\end{table*}

%CONSTRAINED SPOKEN : 
%SPONTANEOUS : We first introduce datasets in which the topics of conversation are either casual, or not pre-specified
%in any way. We refer to these corpora as spontaneous, as we believe they most closely mimic
%spontaneous and unplanned spoken interactions between humans.

%\textbf{SwDA}:
%SPONTANEOUS SPOKEN CORPORA
%Perhaps one of the most influential spoken corpora is the Switchboard dataset (Godfrey et al.,
%1992). This dataset consists of approximately 2,500 dialogues from phone calls, along with wordby-word transcriptions with about 500 total speakers. A computer-driven robot operator system
%introduced a topic for discussion between two participants, and recorded the resulting conversation.
%About 70 casual topics were provided, of which about 50 were frequently used. The corpus was
%originally designed for training and testing various speech processing algorithms; however, it has
%since been used for a wide variety of other tasks, including the modeling of dialogue acts such as
%‘statement’, ‘question’, and ‘agreement’ (Stolcke et al., 2000). \\

%\textbf{Loqui:  CONSTRAINED SPOKEN CORPORA}
%The Loqui Human-Human Dialogue Corpus (Passonneau and Sachar, 2014) consists of annotated transcriptions of telephone interactions between patrons and librarians at New York City’s
%Andrew Heiskell Braille & Talking Book Library in 2006. It stands out as it has annotated discussion topics, question-answer pair links (adjacency pairs), dialogue acts, and frames (discourse
%units).\\

%\textbf{MRDA  CONSTRAINED SPOKEN CORPORA}Similarly, the The ICSI Meeting Recorder Dialog Act (MRDA) Corpus(Shriberg et al., 2004)
%has annotated dialogue acts, question-answer pair links (adjacency pairs), and dialogue hot spots5
%.
%It consists of transcribed recordings of 75 ICSI meetings on several classes of topics including: the
%ICSI meeting recorder project itself, automatic speech recognition, natural language processing and
%neural theories of language, and discussions with the annotators for the project.

%\textbf{MELD - Sentiment}:


%\textbf{MELD - DA}:

%\textbf{bt-Oasis}


%\subsection{Emotion/Sentiment Datasets}


%\textbf{Semaine  CONSTRAINED SPOKEN CORPORA}
%The SEMAINE Corpus (McKeown et al., 2010) consists of 100 ‘emotionally coloured’ conversations. Participants held conversations with an operator who adopted various roles designed to
%evoke emotional reactions. These conversations were recorded with synchronous video and audio
%devices. Importantly, the operators’ responses were stock phrases that were independent of the content of the user’s utterances, and only dependent on the user’s emotional state. This corpus motivates
%building dialogue systems with affective and emotional intelligence abilities, since the corpus does
%not exhibit the natural language understanding that normally occurs between human interlocutors. \\


==> experiments.tex <==
This section gathers experiments performed on the \texttt{SILICONE} benchmark. 
We first analyse an appropriate choice for the decoder, which is selected over a set of experiments on our baseline encoders: a pre-trained BERT model and a hierarchical RNN-based encoder ($\mathcal{H}\mathcal{R}$).
%It is structured as follow: first, we start by choosing the decoder we will use to compare the pretrained encoder with the baseline encoders (e.g. pretrained encoder models and hierarchical recurrent encoders). 
Since we focus on small-sized pre-trained representations, we limit the sizes of our pre-trained models to \texttt{TINY} and \texttt{SMALL} (see \autoref{tab:model_size}). We then study the results of the baselines and our hierarchical transformer encoders ($\mathcal{H}\mathcal{T}$) on \texttt{SILICONE} along three axes: the accuracy of the models, the difference in performance between the \texttt{E/S} and the \texttt{DA} corpora, and the importance of pre-training.
As we aim to obtain robust representations, we do not perform an exhaustive grid search on the downstream tasks.
\subsection{Decoder Choice}
Current research efforts focus on single label prediction, as it seems to be a natural choice for sequence labelling problems (\autoref{ssec:notations}).
Sequence labelling is usually performed with CRFs \cite{crf_chen, crf_kumar} and GRU decoding \cite{colombo2020guiding}, however, it is not clear to what extent inter-label dependencies are already captured by the contextualised encoders, and whether a plain MLP decoder could achieve competitive results.
As can be seen in \autoref{tab:baseline}, we found that in the case of \texttt{E/S} prediction there is no clear difference between CRFs and MLPs, while GRU decoders exhibit poor performance, probably due to a lack of training data.
It is also important to notice, that training a sequential decoder usually requires thorough hyper-parameter fine-tuning.
As our goal is to learn and evaluate general representations that are decoder agnostic, in the following, we will use a plain MLP decoder for all the models compared.
\begin{table}[]
\begin{center}
 \resizebox{.4\textwidth}{!}{\begin{tabular}{ c |c c c } 
 \hline
 &Avg  & Avg \texttt{DA} &   Avg \texttt{E/S} \\ \hline
BERT (+MLP) & 72,8& 81.5  & 64.0 \\
BERT (+GRU) &69.9& 80.4 & 59.3 \\ 
BERT (+CRF) &72.8&81.5 & 64.1   \\ \hline
$\mathcal{H}\mathcal{R}$ (+MLP)  &69.8&  79.1 & 60.4   \\
$\mathcal{H}\mathcal{R}$ (+GRU) &67.6& 79.4& 55.7   \\
$\mathcal{H}\mathcal{R}$ (+CRF) & 70.5&80.3 & 60.7   \\
\end{tabular}}
\caption{Experiments comparing decoder performances. Results are given on \texttt{SILICONE} for two types of baseline encoders (pre-trained BERT models and hierarchical recurrent encoders $\mathcal{H}\mathcal{R}$).}\label{tab:baseline}
\end{center}
\end{table}
% Prepare an intorduction to subsection. 
\begin{table*}
\setlength{\tabcolsep}{4pt}
\begin{center}
 \resizebox{\textwidth}{!}{
 \begin{tabular}{c || c || c c c  c c | c c c c c } 
 \hline
 & \textbf{Avg} & \texttt{SwDA}  & \texttt{MRDA} & $\texttt{DyDA}_{\texttt{DA}}$ &$\texttt{MT}$ & $\texttt{Oasis}$  &  $\texttt{DyDA}_\texttt{e}$  & $\texttt{MELD}_s$  & $\texttt{MELD}_\texttt{e}$ & $\texttt{IEMO}$ & $\texttt{SEM}$ \\ \hline
    BERT-4layers& 70.4 & 77.8 & 90.7  & 79.0 &88.4 & 66.8 & 90.3 & 55.3  &53.4 & 43.0 &58.8\\
    BERT& 72.8 & 79.2  &90.7  & \textbf{82.6} & 88.2   &66.9& 91.9 & 59.3  &\textbf{61.4} & \textbf{45.0} &62.7\\
     $\mathcal{H}\mathcal{R}$& 69.8 & 77,5  &90,9 & 80,1 & 82,8 & 64,3 & 91.5 &59,3 & 59.9 & 40.3& 51.1 \\
     $\mathcal{H}\mathcal{T}(\theta_{MLM}^{u,d})_{\texttt{(TINY)}}$ &73.3& \textbf{79.3}  &92.0& 80.1 & 90.0   &68,3  & 92.5 &62.6 & 59.9 &42.0&66.6\\
     $\mathcal{H}\mathcal{T}(\theta_{GAP}^{d})_{\texttt{(TINY)}}$ & 71.6 & 78.6  & 91.8 & 78.1 & 89.3   & 64.1 & 91.6 & 60.5 & 55.7 & 42.2 & 63.9 \\
    $\mathcal{H}\mathcal{T}(\theta_{MLM}^{u,d})_{\texttt{(SMALL)}}$ & \textbf{74.3} & 79.2  & \textbf{92.4}& 81.5 & \textbf{90.6}   &\textbf{69.4}  & \textbf{92.7} & \textbf{64.1} &60.1& \textbf{45.0} & \textbf{68.2}
\end{tabular}
}
\caption{Performances of different encoders when decoding using a MLP on \texttt{SILICONE}. The datasets are grouped by label type (\texttt{DA} vs \texttt{E/S}) and ordered by decreasing size. $\texttt{MT}$ stands for $\texttt{Map Task}$, $\texttt{IEM}$ for $\texttt{IEMOCAP}$ and $\texttt{Sem}$ for $\texttt{Semaine}$.}
\label{tab:results}
\end{center}
\end{table*}

\subsection{General Performance Analysis}
\autoref{tab:results} provides an exhaustive comparison of the different encoders over the \texttt{SILICONE} benchmark.
As previously discussed, we adopt a plain MLP as a decoder to compare the different encoders.
We show that \texttt{SILICONE} covers a set of challenging tasks as the best performing model achieves an average accuracy of $74.3$.
Moreover, we observe that despite having half the parameters of a BERT model, our proposed model achieves an average result that is $2\%$ higher on the benchmark.
%\subsection{\texttt{DA} and \texttt{E/S} prediction}
\texttt{SILICONE} covers two different sequence labelling tasks: \texttt{DA} and \texttt{E/S}.
In \autoref{tab:results} and \autoref{tab:baseline}, we can see that all models exhibit a consistently higher average accuracy (up to $14\%$) on \texttt{DA} tagging compared to \texttt{E/S} prediction. This performance drop could be explained by the different sizes of the corpora (see \autoref{tab:presentation_of_silicon}). 
%This phenomenon can not be entirely explained by the size of datasets: \texttt{E/S} datasets have smaller size (aside from $\texttt{DyDA}_\texttt{e}$) compared to Dialog Act datasets as reported in \autoref{tab:presentation_of_silicon}.
Despite having a larger number of utterances per label ($u/l$), \texttt{E/S} tasks seem generally harder to tackle for the models. For example, on \texttt{Oasis}, where the $u/l$ is inferior than those of most \texttt{E/S} datasets ($\texttt{MELD}_\texttt{s}$, $\texttt{MELD}_\texttt{e}$, \texttt{IEMO} and \texttt{SEM}), models consistently achieve better results.
%around $64,1\%$ to $69.4\%$ versus $42\%$ to $68.2$.
%While considering, the number of utterances per label we hypothesise that \texttt{E/S} are harder to learn than \texttt{DA}, for the considered models. For example, on \texttt{Oasis}, which has smaller number of utterances per label ($u/l$) compared to \texttt{E/S} dataset (e.g. $\texttt{MELD}_\texttt{s}$, $\texttt{MELD}_\texttt{e}$, \texttt{IEMO} and \texttt{SEM}), models achieve better results around $64,1\%$ to $69.4\%$ versus $42\%$ to $68.2$. 
%Nevert Intuitively, we believe that dialogue act prediction is more related to text modality only when an utterance can be expressed with different emotion and sentiment regarding to other modality values such as speech or face expression.
 
\subsection{Importance of Pre-training for \texttt{SILICONE}} %hierarchical model achieves better results on $SILICONE$}
Results reported in \autoref{tab:results} and \autoref{tab:baseline} show that pre-trained transformer-based encoders achieve consistently higher accuracy on \texttt{SILICONE}, even when they are not explicitly considering the hierarchical structure.
%While, comparing models using a limited number of parameters (see \autoref{tab:model_size}), such as the model with \texttt{TINY} size, using hierarchical pretraining with a BERT model with 4 layers shows a consistent improvement. \\
This difference can be observed both in small-sized datasets (e.g. \texttt{MELD} and \texttt{SEM}) and in medium/large size datasets (e.g \texttt{SwDA} and \texttt{MRDA}).
To validate the importance of pre-training in a regime of low data, we train different $\mathcal{H}\mathcal{T}$ (with random initialisation) on different portions of \texttt{SEM} and $\texttt{MELD}_\texttt{s}$.
Results shown in \autoref{fig:exp_split_semaine} illustrate the importance of pre-trained representations.
\begin{figure}
  \centering
  \includegraphics[width=0.45\textwidth]{schema/exp_split_semaine.pdf}
    \caption{A comparison of pre-trained encoders being fine-tuned on different percentage the training set of \texttt{SEM}. Validation and test set are fixed over all experiments, reported scores are averaged over 10 different random split.}
    \label{fig:exp_split_semaine}
\end{figure}

==> section2_backup.tex <==
\subsection{Notations}\label{ssec:notations}
We start by formally defining the Sequence Labelling Problem. At the higher level, we have a set $D$ of conversations composed of utterances, i.e $D = (C_1,C_2,\dots,C_{|D|})$ with $Y= (Y_1,Y_2,\dots,Y_{|D|})$ the corresponding set labels (e.g. emotions, das). At a lower level each conversation $C_i$ is composed of utterances $u$, i.e $C_i= (u_1,u_2,\dots,u_{|C_i|})$ with $Y_i = (y_1, y_2, \dots, y_{|C_i|})$ the corresponding sequence of labels: each $u_i$ is associated with a unique label $y_i$. At the lowest level, each utterance $u_i$ can be seen as a sequence of words, i.e $u_i = (\omega^i_1, \omega^i_2, \dots, \omega^i_{|u_i|})$. 

\subsection{Related Work}
% on commence avec les transformer mais pas trop transformer + hierarchy textbf{(Chloe) dialog or multi-utterance spontaneous speech?} 
Sequence labelling problems for spoken dialog mainly relies on two different types of labels: emotions or sentiment and dialog acts. Although, early work has tackled the sequence labelling problem as an independent classification of each utterance the current SOTA deep neural networks \cite{bayesian_dialog,svm_dialog,hmm_dialog} model both contextual dependencies between utterances \cite{colombo2020guiding,concurrent_mrda} and labels \cite{crf_chen,crf_kumar,crf_li}.

Aforementioned algorithms make use of large corpora such as Switchboard Dialog Act (SwDA) \cite{datase_swda},  Meeting Recorder Dialog Act (MRDA) \cite{dataset_mrda}, Daily Dialog Act \cite{dataset_dailydialog}, HCRC Map Task Corpus (MapTask) \cite{dataset_maptask} to learn a new model from scratch, making harder the adaptation to smaller dataset such as Loqui human-human dialogue corpus (Loqui) \cite{dataset_loquihuman}, BT Oasis Corpus (Oasis) \cite{dataset_gtoasis}, Multimodal Multi-Party Dataset (MELD) \cite{dataset_meld}, Interactive emotional dyadic motion capture
database (IEMOCAP) , SEMAINE \cite{dataset_semaine}. Despite the variety of labelled datasets, sequence labeller are usually evaluated on a limited number of datasets. SILICONE is the first benchmark to gather such a diversity of corpora.

Some pioneer works take inspiration from recent NLU success in pretraining objectives to attempt to learn spoken dialog task agnostic representation \cite{mehri2019pretraining,emotion_transfert} but the size of collected datasets is limited \cite{ubuntu,multiwoz}. 



%\textbf{(CHloe) dialogue level or multi-utterance level ? Caracteristiques specifiques du dialogue : le dialogue est une sequence de tours de parole avec des locuteurs differents. Chaque tour de parole contient une séquence de phrases.}

\subsection{Pretrained Language Models}
In this section we start by reviewing the two pretraining objectives our work is based on: Masked Language Model (MLM)  from \citet{bert,roberta,albert} and the Generalized Autoregressive Pretraining (GAP) from \citet{xlnet}. 

\textbf{Notations}: Given an input utterance $u_i$ composed of words or subwords  $u_i = (\omega^i_1, \omega^i_2, \dots, \omega^i_{|u_i|})$, Transformer based architectures trains an encoder that produces a contextualised vector representation for each unit: $enc(\omega^i_1, \omega^i_2, \dots, \omega^i_{|u_i|}) = (x_1, x_2, . . . , x_{|u_i|})$.

\textbf{MLM}: is the task of predicting a subset of missing token in a sentence. Formally, a random set of index position $m^{u_i}$ is selected and associated token are replaced by a masked token [MASK] to obtained a corrupted utterance $u^\text{masked}_i$. The model with parameter $\theta$ is learnt by maximising : 
\begin{equation}
     \mathcal{L}_{MLM}(\theta,u_i)=\mathbb{E}\big(\sum_{t \in m^{u_i}} \log(p_{\theta}(\omega^t | u^\text{masked}_i)\big)
\end{equation}

\textbf{GAP}: contrarily to MLM allows to maximise the expected log likelihood across all permutation orders and do not use any input corruption. The GAP loss can be written as:
\begin{equation}
\mathcal{L}_{GAP}(\theta,u_i) = \mathbb{E}_{\textbf{z} \sim \mathbb{Z}_|u_i|} \bigg[ \sum_{t} \log p_{\theta}(\omega^{z_t} | u_i^{{\textbf{z}<t}})\bigg]
\end{equation}
where $\mathbb{Z}_{|u_i|}$ is the set of all permutations of size $|u_i|$.

\textbf{Multi-Task Losses for LMs}: are used by \citet{hierarchy_loss,garcia2019token} to introduce an inductive bias by supervising a set of low level tasks at the bottom layers of the model and more complex tasks at the highest layers of the model.

%\textbf{(CHloe) dialogue level or multi-utterance level ? Caracteristiques specifiques du dialogue : le dialogue est une sequence de tours de parole avec des locuteurs differents. Chaque tour de parole contient une séquence de phrases.}



==> structure.tex <==


\section{Methods}
\subsection{Background}
Notation
pretrained language model
Background on multi-loss
%%% Method presentation
\subsection{Hierarchical Encoding}
dialog => then pretrained 

\subsection{Hierarchical Pretraining}

\subsection{Baseline Encoder}

\subsection{Pretraining Datasets}
%%%% 
\section{Evaluation of SL}
\subsection{Background}

\subsection{\texttt{SILICONE}}

==> tasks.tex <==
In this section we describe pretraining corpus as well as downstream tasks composing the benchmark.

\subsection{Choice of Pretraining Dataset}
In our work we focus on \textit{OpenSubtitles} \cite{opensub} \footnote{http://opus.nlpl.eu/OpenSubtitles-alt-v2018.php} because (1) it contains spoken language, contrarily to the Ubuntu corpus \cite{ubuntu} based on logs, and (2) as Wizard of Oz \cite{multiwoz} and  Cornell Movie Dialog Corpus \cite{cornell}, it is a multi-party dataset, but is an order of magnitude larger. After pre-processing Opensubtitles contains subtitltes from $446520$ movies or series which represent $54642424$ conversations and over $2.3$ billion of words. 


%There exists few datasets that are freely available f
%Although there exist some dataset that contains 
%To the best of our knowledge, there exists few datasets t suitable for pretraining a langage model for spoken conversations.
%\begin{itemize}
%    \item \textit{Cornell Movie Dialog Corpus}\cite{cornell}
%    \item \textit{Ubuntu Dialog Corpus}\cite{ubuntu}
%    \item \textit{Wizard of Oz}\cite{multiwoz}
%    \item \textit{Opensubtitles}\cite{opensub}
%\end{itemize} 

%\textit{Cornell Movie Dialog Corpus} way too small and conversations are not long enough, \textit{Ubuntu} based on logs i.e written language and we studie spoken language. Both datasets contains bi-party conversation which can be a limitation as we want a more universal system.
%On the contrary \textit{Wizard of Oz} is a multi-party dataset but too small.\\
%Thus we focused on the \textit{Opensubtitles} corpus \footnote{http://opus.nlpl.eu/OpenSubtitles-alt-v2018.php}, the only corpus from spoken language and large enough to train transformer based model. corpus\cite{opensub}. It contains subtitltes from $446520$ movies or series which represent $54642424$ conversations and $273212120$ fragment of sentences.



\subsection{Benchmark Presentation}
We introduce \texttt{SILICONE} a collection of sequence labelling tasks including dialog act, sentiment and emotion labels. SILICONE does not place any constraints on model architecture beyond the ability to process multiple sequence inputs and to make corresponding predictions of the desired label. SILICONE was not created from scratch; it relies on preexisting datasets because they have been agreed upon by the community as challenging and interesting. Considered datasets  have different tag sets depending on the annotation schema (e.g. DIT++ \cite{bunt2009dit++} and DAMSL \cite{damsl} for \texttt{DA}). Additionally, some corpora (\textit{e.g} \texttt{MRDA}, \texttt{SwDA}) are manually segmented \cite{3,4} (hence segmentation depends on the perspective of the transcriber) whereas other corpora (\textit{e.g.} \texttt{SEMAINE}) rely on automatic solutions \cite{5}. We design the benchmark such that good performance should require a model to have substantial knowledge and could adapt to small size dataset. Evaluating with different tag sets of different size gives valuable insight into the model generalisation. Dataset composing the benchmark are introduced based on their size and can be found in the following sections and statistics are gathered in \autoref{tab:presentation_of_silicon}. 



%contains small and large dataset

%As our pretraining task on OpenSubtitle aims at resulting in representation that are label-agnostic and can be fine-tuned it is critical to develop a new benchmark on which we can compare the different models. We introduce SILICONE a collection of sequence labelling tasks including dialog act, sentiment and emotion labels. SILICONE does not place any constraints on model architecture beyond the ability to process multiple sequences inputs and to make corresponding predictions of the desired label. SILICONE was not created from scratch; it relies on preexisting datasets because they have been agreed upon by the community as challenging and interesting. We design the benchmark such that good performance should require a model to have substantial knowledge and could adapt to small size dataset. 

%\textbf{Miscellous}
%Additionnal ideas, transfert learning task specifics, different sizes Underly the fact that we use corpus of different size. , split follow


\subsubsection{Dialog Act Datasets}
\textbf{Switchboard Dialog Act Corpus ($SwDA$)}: is a telephone speech corpus consisting  of two-sided telephone conversation with provided topics. This dataset includes additional features such as speaker id and topic information usually used in SOTA models. SOTA models report an accuracy of $85.5\%$ \cite{colombo2020guiding} on the official split and make use of Seq2seq models with augmented training and inference mechanism such as guided attention, beam search at training and inference and a huge grid search. \\
\textbf{ICSI MRDA Corpus ($MRDA$)} has been introduced by \citet{dataset_mrda}. It contains transcripts of multi-party meetings hand-annotated with DAs. It is the second biggest dataset with arround $110k$ utterances. SOTA models reaches an accuracy of $92.2\%$ \cite{sota_swda_1} and use Bi-LSTM with attention as encoder as well as additional features such as Topic. \\   
\textbf{DailyDialog Act Corpus ($DyDA_a$)}: has been produced by \citet{dataset_dailydialog} contains multi-turn dialogues and is a human-written dialog. It is supposed to reflect our daily communication and so covers topics about our daily life. The dataset is manually labelled with dialog act and emotions. It is the third biggest corpus of SILICON with $102k$ utterances. SOTA models report an accuracy of $88.1\%$ \cite{sota_swda_1} use a Bi-LSTM with attention as well as additional features such as Topic. We follow the official split introduced by the authors. \\
\textbf{HCRC MapTask Corpus ($MapTask$)}: has been introduced by \cite{dataset_maptask}. To build this corpus participants were asked to collaborate verbally by describing a route on one of the participant’s map on the map of another participant. This corpus is small ($27k$ utterances). As there is no standard train/dev/test split\footnote{We split according to the code in https://github.com/NathanDuran/Maptask-Corpus. SILICONE will contain our split.} performances depends on the split. \cite{tran2017generative} make use of Hierarchical LSTM encoder with a GRU decoder layer. \\
\textbf{Bt Oasis Corpus ($Oasis$)} contains the transcripts of live calls made to the BT and operator services. This corpus has been introduced by \cite{dataset_gtoasis} and is rather small ($15k$ utterances). There is no standard train/dev/test split \footnote{We use a random split from https://github.com/NathanDuran/BT-Oasis-Corpus. SILICONE will contain our split.} and few work has been conducted on this dataset. 

\subsubsection{Sentiment/Emotion Datasets}
In Sentiment/Emotion recognition for spoken language there is a high variability both in the preprocessing step for labels and for the choice of the evaluation metric. (e.g \citet{weighted_preproc,weighted_no} use a weighted F-score where \citet{accuracy_fscore} report accuracy). For SILICONE we choose to stay consistent with the current trend in DA research and thus follow \citet{accuracy_fscore} and report the accuracy. Additionally emotion/sentiment labels are not merged and not preprocessed. \\
\textbf{DailyDialog Emotion Corpus ($DyDA_e$)}: This dataset has been previously introduced and contains emotion annotation as well. SOTA model \cite{de2019joint} make use of a BERT with additional Valence Arrousal and Dominance features and reach an accuracy of 85\% on the official split. \\
\textbf{Multimodal EmotionLines Dataset ($MELD$):} has been created by enhancing and extending EmotionLines dataset \cite{emotion_lines} where multiple speakers participated in the dialogues. There are two types of annotations $MELD_s$ and  $MELD_e$: sentiments (positive, negative and neutral) and seven emotions (anger, disgust, fear, joy,neutral, sadness and surprise). $MELD$ is a small size dataset and we follow the official split introduced by the authors. SOTA model with text only is proposed by \citet{accuracy_fscore} and is inspired by quantum physics. In their work, they compare also to a hierarchical bi-LSTM and report an accuracy of $60.8\%$ ($MELD_s$) and $65.2$ ($MELD_e$) against $61.9$\% and $67.9$\% for their model. \\
\textbf{IEMOCAP database ($IEMOCAP$):} is a multimodal database of ten speakers. It consists of dyadic sessions where actors perform improvisations or scripted scenarios. Emotion categories are: anger, happiness, sadness, neutral, excitement, frustration, fear, surprise, and other. There is no official split on this dataset proposed models are built bi-LSTM and achieves $35.1\%$ with text only \cite{accuracy_fscore}. \\
\textbf{SEMAINE database ($SEMAINE$)} comes from the Sustained Emotionally coloured Machine human Interaction using Nonverbal Expression project \cite{dataset_semaine} and has three sentiments labels (positive, negative and neutral) . It is build on Multimodal Wizard of Oz experiment where participants held conversations with an operator who adopted various roles designed to evoke emotional reactions. There is no official split on this dataset.\\

\begin{table*}
\begin{center}
 \begin{tabular}{c c c c c c c c c} 
 \hline
 Corpus & Domain  & $\lvert Train \rvert$ & $\lvert Val \rvert$ & $\lvert Test \rvert$ & Utt.& $\lvert Labels \rvert$ &Task& Utt./\lvert Labels \rvert \\ 
  \hline
  $SwDA$\footnote{For these datasets we follow the official split train/test} & Open &  1k  & 100 & 11 & 200k   & 42 & \texttt{DA} & 4.8k\\

  $MRDA$\footnotemark[\value{footnote}] & Meetings & 56 & 6 &  12 &110k& 5& \texttt{DA} & 2.6k\\
      $DyDA_a$& Daily Life &  11k  & 1k & 1k & 102k  & 4 & \texttt{DA}& 25.5k \\
  $MapTask$\footnotemark[\value{footnote}] & Routes & 121 & 22 & 25 &  36k & 12& \texttt{DA} & 3k\\
  $Oasis$\footnotemark[\value{footnote}] & Customers calls& 508 & 64 & 64 & 15k & 42 & \texttt{DA} & 357\\
 \hline
    $DyDA_e$ & Daily Life &  11k  & 1k & 1k & 102k  & 7 &\texttt{E}&2.2k \\
    $MELD_s$ & Movie & 934 & 104  &  280 & 13k  & 3 & Sent & 4.3k\\
        $MELD_e$ \footnotemark[\value{footnote}]& Movie & 934 & 104  &  280 & 13k  & 7 & \texttt{E} & 1.8k\\
    $IEMOCAP$& \multirow{2}{*}{ \makecell{ Emotional \\ conversations}} & 108 & 12 & 31 & 10k & 6 & \textit{Em.}&1.7k\\

      $SEMAINE$ & & 62 & 7 & 10 & 5,6k &3 & Sent.& 1.9k\\

\end{tabular}
\label{tab:presentation_of_silicon}
\caption{Statistics of datasets composing $SILICONE$. \textit{Em.} stands for emotion label and Sent. for sentiment label; \footnotemark[\value{footnote}] stands for datasets with available official split.}
\end{center}
\end{table*}

%CONSTRAINED SPOKEN : 
%SPONTANEOUS : We first introduce datasets in which the topics of conversation are either casual, or not pre-specified
%in any way. We refer to these corpora as spontaneous, as we believe they most closely mimic
%spontaneous and unplanned spoken interactions between humans.

%\textbf{SwDA}:
%SPONTANEOUS SPOKEN CORPORA
%Perhaps one of the most influential spoken corpora is the Switchboard dataset (Godfrey et al.,
%1992). This dataset consists of approximately 2,500 dialogues from phone calls, along with wordby-word transcriptions with about 500 total speakers. A computer-driven robot operator system
%introduced a topic for discussion between two participants, and recorded the resulting conversation.
%About 70 casual topics were provided, of which about 50 were frequently used. The corpus was
%originally designed for training and testing various speech processing algorithms; however, it has
%since been used for a wide variety of other tasks, including the modeling of dialogue acts such as
%‘statement’, ‘question’, and ‘agreement’ (Stolcke et al., 2000). \\

%\textbf{Loqui:  CONSTRAINED SPOKEN CORPORA}
%The Loqui Human-Human Dialogue Corpus (Passonneau and Sachar, 2014) consists of annotated transcriptions of telephone interactions between patrons and librarians at New York City’s
%Andrew Heiskell Braille & Talking Book Library in 2006. It stands out as it has annotated discussion topics, question-answer pair links (adjacency pairs), dialogue acts, and frames (discourse
%units).\\

%\textbf{MRDA  CONSTRAINED SPOKEN CORPORA}Similarly, the The ICSI Meeting Recorder Dialog Act (MRDA) Corpus(Shriberg et al., 2004)
%has annotated dialogue acts, question-answer pair links (adjacency pairs), and dialogue hot spots5
%.
%It consists of transcribed recordings of 75 ICSI meetings on several classes of topics including: the
%ICSI meeting recorder project itself, automatic speech recognition, natural language processing and
%neural theories of language, and discussions with the annotators for the project.

%\textbf{MELD - Sentiment}:


%\textbf{MELD - DA}:

%\textbf{bt-Oasis}


%\subsection{Emotion/Sentiment Datasets}


%\textbf{Semaine  CONSTRAINED SPOKEN CORPORA}
%The SEMAINE Corpus (McKeown et al., 2010) consists of 100 ‘emotionally coloured’ conversations. Participants held conversations with an operator who adopted various roles designed to
%evoke emotional reactions. These conversations were recorded with synchronous video and audio
%devices. Importantly, the operators’ responses were stock phrases that were independent of the content of the user’s utterances, and only dependent on the user’s emotional state. This corpus motivates
%building dialogue systems with affective and emotional intelligence abilities, since the corpus does
%not exhibit the natural language understanding that normally occurs between human interlocutors. \\

